Queue Length Simulation for Signalized Arterial Networks and Steady State Computation under Fixed Time Control

We consider traffic flow dynamics for a network of signalized intersections, where the outflow from every link is constrained to be equal to a given capacity function if the queue length is positive, and equal to the minimum of cumulative inflow and capacity function otherwise. In spite of the resulting dynamics being discontinuous, recent work has proved existence and uniqueness of the resulting queue length trajectory if the inter-link travel times are strictly bounded away from zero. The proof, which also suggests a constructive procedure, relies on showing desired properties on contiguous time intervals of length equal to the minimum among all link travel times. We provide an alternate framework to obtain queue length trajectories by direct simulation of delay differential equations, where link outflows are obtained from the provably unique solution to a linear program. Existence and uniqueness of the solution to the proposed model for traffic flow dynamics is established for piecewise constant external inflow and capacity functions, and the proposed method does not require travel times to be bounded away from zero. Additionally, if the external inflow and capacity functions are periodic and satisfy a stability condition, then there exists a globally attractive periodic orbit. We provide an iterative procedure to compute this periodic orbit. A periodic trajectory is iteratively updated for every link based on updates to a specific time instant when its queue length transitions from being zero to being positive. The update for a given link is based on the periodic trajectories computed in the previous iteration for its upstream links. The resulting iterates are shown to converge uniformly monotonically to the desired periodic orbit.

==> existence-uniqueness-backup.tex <==
\subsection{Existence of Solution to \eqref{eq:flow-dynamics}}
We start by showing uniqueness of the solution obtained from Algorithm~\ref{alg:z-computation-new}. The proof of the next result is provided in the Appendix.

%\begin{proposition}
%\label{prop:solution-properties}
%Given $x \in \real_+^{\mc E}$, $t \geq 0$, $\lambda(t)$, $c(t)$, $\{z(s): s \in [t-\bar{\delta}, t)\}$, and $\mc E_0^{\text{temp}} \subseteq \mc E$, \eqref{z-linprog} has a unique solution, which is independent of $\eta \in \real_{>0}^{\mc E}$. Moreover, the optimal solution satisfies $z_i = c_i(t)$ for all $i \in \mc E \setminus \mc E_0^{\text{temp}}$.
%\end{proposition}

\begin{proposition}
\label{prop:solution-properties}
Given $x \in \real_+^{\mc E}$, $t \geq 0$, $\lambda(t)$, $c(t)$, $\{z(s): s \in [t-\bar{\delta}, t)\}$, \eqref{z-linprog} has a unique solution, which is independent of $\eta \in \real_{>0}^{\mc E}$. Moreover, the optimal solution satisfies 
\begin{equation}
\label{eq:z-def}
z_i(x,t) = \begin{cases} \lambda_i(t) + \sum_{j \in \mc E: \, \delta_{ji}>0} R_{ji} z_j(t-\delta_{ji}) + \sum_{j \in \mc E: \, \delta_{ji}=0} R_{ji} z_j(x,t) & i \in \mc E_0(x,t)   \\
c_i(t) &  i \in \mc E \setminus \mc E_0(x,t)
\end{cases}
\end{equation}
%$z_i(x,t) = c_i(t)$ for all $i \in \mc E \setminus \mc E_0(x,t)$.
\end{proposition}

Proposition~\ref{prop:solution-properties} implies that $z(x(t),t)$ in \eqref{eq:flow-dynamics} is well-defined. 
%Moreover, Algorithm~\ref{alg:z-computation-new} ensures that continuous flow is \emph{possible} from every $x(t)$ under \eqref{eq:flow-dynamics}. 
However, the existence of solution to \eqref{eq:flow-dynamics} depends on the \emph{jumps} in $\mc E_0(x(t),t)$: a jump occurs at time $t>0$ if $\mc E_0(x(t^-),t^-) \neq \mc E_0(x(t),t)$. This in general depends on $\lambda(t)$ and $c(t)$. The next result, whose proof is provided in the Appendix, gives a sufficient condition for the existence of solution to \eqref{eq:flow-dynamics}.

\ksmargin{could there be infinite number of switches in $z$ due to 'feedback' effect under delay ?}
\begin{proposition}
\label{prop:existence-traffic-dynamics-solution}
If $c(t)$ and $\lambda(t)$ are piecewise constant, then there exists a unique solution to \eqref{eq:flow-dynamics} for every initial condition $x_0 \in \real_+^{\mc E}$ and \kscomment{$\{z(s): s \in [-\underline{\delta},0)\}$}. \kscomment{Moreover, such a solution satisfies $x(t) \geq 0$ for all $t \geq 0$.}
\end{proposition}

\begin{remark}
\begin{enumerate}
\item \eqref{eq:flow-dynamics} allows direct simulation of queue length dynamics under fixed-time control. Moreover, unlike \cite{Muralidharan.Pedarsani.ea:15}, existence of a unique solution to \eqref{eq:flow-dynamics} does not require $\underline{\delta}$ to be strictly greater than zero. However, this comes at the expense of piecewise constant assumption on the external inflow and capacity functions.  
\item The piecewise constant assumption is practically justified because a common model for a capacity function is such that it is equal to the saturated capacity during the green phase and zero otherwise, and external inflows can be modeled as a sequence of rectangular pulses modeling vehicle platoons.
\kscomment{\item Proposition~\ref{prop:existence-traffic-dynamics-solution} holds true also when the capacity function is state-dependent (referred to as \emph{adaptive} traffic signal control), but piecewise constant.
For example, let the capacity function $c_i(t)$ be equal to  $c_i^{\text{max}}$
if $t \in [\theta_i,\theta_i+g_i(0)] \cup [T+\theta_i, T+ \theta_i + g_i(1)] \cup \ldots$, and equal to zero otherwise, where $\theta_i \in [0,T]$ is the offset, and $\{g_i(0), g_i(1), \ldots\}$ is a sequence of green times. Such green times can be determined as a function of queue lengths. One such simple \emph{proportional} rule, when the capacity functions for all the incoming links at every intersection are mutually exclusive, is:
$$
g_i(k) = \frac{\|x_i(k-1:k)\|_{\infty}}{\sum_j \|x_j(k-1:k)\|_{\infty}}, \qquad k = 1, 2, \ldots
$$
The summation in the denominator is over all links incoming to the intersection to which $i$ is incident, and $\|x_i(k-1:k)\|_{\infty}:=\max_{t \in [(k-1)T,kT]} x_i(t)$ is the maximum queue length during the $k$-th cycle on link $i$.
}
%\item The piecewise constant assumption in Proposition~\ref{prop:existence-traffic-dynamics-solution} is reasonable considering that standard capacity functions are of on/off nature representing alternating green/red phases, and the traffic flow between queues is typically modeled as  \kscomment{rectangular platoons}. 
\end{enumerate}
\end{remark}


%While condition (i) in Proposition~\ref{prop:existence-traffic-dynamics-solution} holds true if one uses vertical queue model, condition (ii) is relevant when queue capacity of links are modeled to be unbounded. In the latter case, the travel times depend on the queue length of the downstream link, and the inter-queue travel times may not be necessarily bounded away from zero. However, the fully utility of this aspect in simulating extensions of \eqref{eq:flow-dynamics} for links with finite queue capacity will be pursued in future. For now, part (ii) of the condition in Proposition~\ref{prop:existence-traffic-dynamics-solution} is to interpreted as a preparatory step towards this future extension. Finally, 


%\begin{proposition}
%\label{prop:solution-properties}
%Given $\eta \in \real_{>0}^{\mc E}$, for every $x \in \real_+^{\mc E}$, there exists a unique solution to \eqref{z-linprog}, and it satisfies the following: 
%\begin{equation}
%\label{eq:outflow-expr-compact}
%\begin{split}
%z_i(x,t) & = c_i(t), \, \, i \in \tilde{\mc E}(x), \\ z_i(x,t) & = \lambda_i(t) + \sum_j R_{ji} z_j(x,t-\delta_{ji}), \, \, i \in \mc E \setminus \tilde{\mc E}(x)
%%\sum_{j \in \mc E \setminus \tilde{\mc E}(x)} c_j(t) +  \sum_{j \in \tilde{\mc E}(x)} \lambda_j(t)
%\end{split}
%\end{equation}
%%where $a_j(\beta,q,x) \geq 0$ are $b_j(\beta,q,x) \geq 0$ are each globally Lipschitz continuous in $x$ for every $\beta$ and $q$. In particular, $z_i(x,t)=c_i(t)$ for all $i \in \mc E \setminus \tilde{\mc E}(x)$. Moreover, the vector field given in \eqref{eq:flow-dynamics} is globally Lipschitz continuous for every $q \in \mathbf{Q}$.
%\end{proposition}

%\begin{remark}
%\begin{enumerate}
%\item Proposition~\ref{prop:solution-properties} implies that link outflows, as given by \eqref{eq:outflow-expr-compact}, are independent of the choice of $\eta$.
%\item \kscomment{Note that Proposition~\ref{prop:solution-properties} applies to fixed as well as adaptive control policies.}
%\end{enumerate}
%\end{remark}

==> lit-review.tex <==
\section{Introduction}
\label{sec:lit-review}



We conclude this section by introducing key concepts and notations to be used throughout the paper. $\real$, $\real_{\geq 0}$, $\real_{>0}$, $\real_{\leq 0}$ and $\real_{< 0}$ will stand for real, non-negative real, strictly positive real, non-positive real, and strictly negative real, respectively, and $\NN$ denotes the set of natural numbers. 
%$\complex$ will denote the set of complex numbers. For $x \in \complex$, we let $\bar{x}$ denote its complex conjugate, and let $\Re(x)$ and $\Im(x)$ denote the real and imaginary parts, respectively, of $x$. 
For $x \in \real$, we let $[x]^+=\max \{x,0\}$ denote the non-negative part of $x$. 

The road network topology is described by a directed multi-graph $\mc G=\left(\mc V,\mc E\right)$, where $\mc V$ are the set of intersections and $\mc E$ are the set of directed links. 
The head and tail nodes of a cell $i$ are denoted by $\tau_i$ and $\sigma_i$, respectively, so that the cell $i=(\sigma_i,\tau_i)$ is directed from $\sigma_i$ to $\tau_i$.
Let $T>0$ be the common cycle time at all the intersections. 
\kscomment{Relevant quantities, e.g., offset, which refer to a specific time inside the cycle are to be interpreted as being modulo $T$.} 
For $v \in \mc V$, let $\mc E_v^+:=\setdef{i \in \mc E}{\sigma_i = v}$ and $\mc E_v^-:=\setdef{i \in \mc E}{\tau_i = v}$ be the set of outgoing and incoming links, respectively, with respect to $v$. 



==> simulations.tex <==
\section{Simulations}
\label{sec:simulations}
\ksmargin{need to fill in details}
Figure~\ref{fig-network} depicts comparison between steady state queue lengths obtained by direct simulation of \eqref{eq:flow-dynamics}-\eqref{z-linprog}, and by the iterative approach proposed in Algorithm~\ref{alg:steady-state-computation-network}, for a sample network comprises 9 signalized intersections and 24 links operating under fixed time controller. All intersections have common cycle time of 20 seconds. $\lambda(t)$ and $c(t)$ of each link are chosen such that the necessary condition is satisfied. Turning ratios at each intersection are defined such that $\sum_{j} R_{ji} =0.9$ for all $j \in \mc E$. We choose the initial condition $x_0=10$ on each link when using the direct simulation to find the steady-state queue lengths.
% \kscomment{The parameters for the simulations are: $T=20$, $\lambda(t)=?$, $c(t)=?$, $R_{ij}=?$, and $x_0=?$. }

%The difference between computed and actual steady state queue lengths values.
%The root mean square error (RMSE) in this table is defined as 
%$$ \frac{ \sum_{t=1}^{T} { (\hat{x}_i(t)-x_i(t))^2 } }{ T }$$ 
%where $x_i(t)$ and $\hat{x}_i(t)$ are the true link volumes and computed ones at time $t$ respectively. 
The RMSE (root mean square error) is defined as follows:
$$\sqrt  {\frac{ \sum_{t=1}^{T} { (\hat{x}_i(t)-x_i(t))^2 } }{ T } }$$ 
where $\hat{x}_i(t)$ and $x_i(t)$ are steady state queue lengths obtained by the proposed iterative approach, and by direct simulation at time $t$ respectively. 

 %The relative error reported in these figures is defined as 
%$\frac{\| \hat{a}-a \|_2}{\|a\|_2}$, where $a$ and $\hat{a}$ are the true vector and estimated vector respectively. %The relative error is computed for $x$, $f$ and the total OD flow in the network.

 The convergence of RMSE to zero illustrates the correctness of Algorithm~\ref{alg:steady-state-computation-network} in computing steady-state queue lengths. Moreover, the monotonically decreasing nature of RMSE errors in queue lengths for all the links illustrates the monotonicity result in Proposition~\ref{prop:outflow-update-monotonicity}.
% 
%
%The steady state of for the network shown in Figure \ref{fig-network} (a) is computed using the proposed algorithm.
%The network comprises 9 signalized intersections and 24 links and is operating under fixed time policy. All intersections have common cycle time of 20 seconds. Vehicles can arrive on every link. The arrival rates and saturation flow capacities are constant and chosen such that the stability condition is satisfied.
%The root mean square error (RMSE) for representative links is provided in Table \ref{table:error}. Figure \ref{fig:rmse-iterations} shows how fast the computation algorithm converges. 

 %\kscomment{The saturated capacities and the external inflows are given by ... The identical cycle length at all the intersections is given by $T=20$.} \ksmargin{fill in details here}

\begin{figure}
\begin{center}
%\vspace{-0.3in}
\includegraphics[width=1.65 in]{ex1-network.jpg} \hspace{0.1in}
\includegraphics[width=1.5 in]{ex1_link17.pdf} \hspace{0.1in}
\includegraphics[width=2.0 in]{convergence_plot_new.pdf} 
%\includegraphics[width=1.5 in]{/Users/ksavla/papers/2017/Hosseini.Savla.TRB.Journal/results/ex1_link17.pdf} \hspace{0.1in}
%\includegraphics[width=2.0 in]{/Users/ksavla/papers/2017/Hosseini.Savla.TRB.Journal/results/convergence_plot_new.pdf} 
\caption{\small \sf (Left) Graph topology for the network used in the simulations. (Middle) Comparison between steady state queue length obtained from direct solution and from the proposed iterative procedure for link 17. (Right) Evolution of RMSE between steady state queue length from direct simulations and from the proposed procedure for few sample links; the monotonic decrease in RMSE illustrates the monotonic convergence property of the proposed algorithm. 
}%(a) and \ref{sec:offset-opt} (b,c). }
\vspace{-0.3in}
\label{fig-network}
\end{center}
\end{figure}

%\begin{figure}
%\begin{center}
%\includegraphics[width=1.8 in]{ex1-network.jpg} \hspace{0.5in}\\
%\caption{Graph topologies of the networks used in the simulations in Section~\ref{sec:steady-state}. }
%\label{fig-network}
%\end{center}
%\end{figure}

\begin{comment}
\begin{figure}[htb!]
\begin{center}				
\includegraphics[width=1 in]{ex1_link2} 
\includegraphics[width=1 in]{ex1_link10} 
\includegraphics[width=1 in]{ex1_link17} 
\end{center}
 \caption{Comparison of steady state trajectories obtained from the iterations in Section~\ref{sec:steady-state-computation} (top) and by direct simulations (bottom) for links 2 (left), 10 (middle) and 17 (right). Link numbers refer to Figure~\ref{fig:topography}.}
\label{fig:actual-vs-computed}
\end{figure}
\end{comment}
%\ksmargin{fill up details for all links, and take the square root of all the numbers}

 
%\begin{table}[htb!]
%\centering
%\begin{tabular}{|c|c|c|c|c|c|c|l|} \hline
%Link ID& 1 & 2 & 3 & 7& 8 & 9\\ \hline
%RMSE &0.5106  &  0.6042  & 0.1908   & 0.5252   & 0.8312    &  0.5444   \\ \hline   \hline
%Link ID& 14 & 15 & 16 & 21& 22 & 23\\ \hline
%RMSE&1.2830 &0.7123&0.3040& 0.4327 & 0.4043 & 0.3402\\ \hline  
%
%\end{tabular}
%\caption{RMSE between steady-state queue lengths computed using the iterative procedure and by direct simulations.
%}
%\label{table:error}
%\end{table}

%\begin{figure}[htb!]
%\begin{center}				
%\includegraphics[width=3 in]{convergence_plot_1.jpg} 
%\end{center}
% \caption{RMSE between steady-state queue lengths computed using the iterative procedure and by direct simulations versus number of iterations.}
%\label{fig:rmse-iterations}
%\end{figure}

==> steady-state-single-link-finite-capacity.tex <==
\section{Steady State Computation for the Finite Capacity Case}
\label{sec:steady-state-single-link-finite-capacity}

\subsection{The Single Link Case}
\label{sec:finite-capacity-single-link}
\kscomment{In this section, we extend the algorithm from Section~\ref{sec:steady-state-single-link} to the case when the link has finite queue capacity, say $B_i>0$.} In the most basic case, one has to consider two links in series: flows arrive to $i_0$ which has unbounded queue capacity, from which it enters $i$ if $x_i < B_i$. The state of this setup is $(x_{i_0},x_i)$. It suffices to find $(x_{i_0},x_i)$ at a specific time instant. \kscomment{Under the assumption that this setup admits a periodic steady-state}, we provide an extension of Algorithm~\ref{alg:steady-state-computation-single-link}. 

Recall Definition~\ref{def:transition-points}, where the transition points are to be interpreted for the non-virtual link. 
We extend the definition of transition point to also include time instants when the queue length transitions from being at capacity $B_i$ to being less than capacity. Let these points be denoted as $\gamma_i^1, \ldots, \gamma_i^P$. Note that, unlike$L$, $P$ can be zero even if the \kscomment{stability condition} is strictly satisfied. 
Analogous to Proposition~\ref{prop:main-computation}, there exists a strictly increasing $\map{k_{\gamma}}{\until{P}}{\until{M_i^b}}$ such that $\gamma_i^{p} = \underline{b}_i^{k_{\gamma}(p)}$.
%The definition of $\mc W_i^{\alpha}$ needs to be modified as follows. 
%For $t \in [0,T]$, let $z_i(t):=$
Let 
\begin{align*}
\hat{Z}_i(s_1,t) & := Y_i(s_1,t) - C_i(s_1,t), \qquad t \in [s_1,s_2] \\
Z_i(s_1,t) & := \hat{Z}_i(s_1,t) - \sup \setdef{\left[\hat{Z}_i(s_1,s) - B_i \right]^+}{s_1 \leq s \leq t}
\end{align*}

Let $\mc W_i^{\alpha} := \left\{\underline{w}_i^{k_1}, \ldots,  \underline{w}_i^{k_m}\right \}$ be such that $k_1=1$, and, for $j \in \{2, \ldots, m\}$, 
%\begin{equation}
%\label{eq:M-def}
%k_j = \argmin \left \{ind \in \{k_{j-1}+1, \ldots, M^w\} \, \Big | \, [\underline{w}_i^{ind-1},\underline{w}_i^{ind}] \cap \{\underline{b}_i^1, \ldots, \underline{b}_i^{M_i^b}\} \neq \emptyset \right\}
%\end{equation}
%\begin{equation}
\begin{multline}
\label{eq:M-def-finite-capacity}
k_j = \argmin \Big \{ind \in \{k_{j-1}+1, \ldots, M_i^w\} \, \Big | \, \exists \, p \in \until{M_i^b} \text{ s.t. } \bar{b}_i^p \in [\underline{w}_i^{ind-1},\underline{w}_i^{ind}]  \quad \& \\ Z_i(\underline{w}_i^{ind-1},\bar{b}_i^p) \leq 0 \text{ if } \bar{b}_i^p < \underline{w}_i^{ind}, \text{ or } Z_i(\underline{w}_i^{ind-1},\bar{b}_i^p) < 0 \text{ if } \bar{b}_i^p = \underline{w}_i^{ind}\Big \}
\end{multline}
%\end{equation}
where $m$ is implicitly defined to be the maximum value of $k_j$, when the set over which $\argmin$ is taken in \eqref{eq:M-def} is empty. 
With this modification, Proposition~\ref{prop:gamma-1-computation-correctness} holds true, i.e., $\alpha_i^{\ell}=\underline{w}_i^{k_m+\ell-L}$ for all $\ell \in \until{L}$.
Therefore, the procedure to compute periodic orbit can be summarized as follows:
\begin{enumerate}
\item use Algorithm~\ref{alg:steady-state-computation-single-link} to compute periodic orbit $x^*_i$ with inflow function $y_i(t)$, capacity function $c_i(t)$, and the modified definition of $\mc W_i^{\alpha}$ as in \eqref{eq:M-def-finite-capacity}
\item define the saturated capacity function for $i_0$ as follows:
\begin{equation*}
\label{eq:c-virual-link-def}
c_{i_0}(t) = \begin{cases} y_i(t) & x_i^*(t) < B_i   \\
c_i(t) &  x_i^*(t) = B_i
\end{cases}
\end{equation*}
\item use Algorithm~\ref{alg:steady-state-computation-single-link} to compute periodic orbit for the virtual link,  with inflow $y_i(t)$, saturated capacity function $c_{i_0}(t)$, and the definition of $\mc W_i^{\alpha}$ as in \eqref{eq:M-def}.
\end{enumerate}

\subsection{The Network Case}
\label{sec:finite-capacity-network}
We now extend the procedure described in Section~\ref{sec:finite-capacity-single-link} to a network. 
\kscomment{Assume that, for every link, the capacity function associated with the incoming links are mutually exclusive.}

Algorithm~\ref{alg:steady-state-computation-network} extends to an acyclic network, with modification to $\mc F_x$ and $\mc F_z$ as follows. Acyclicity implies a topological ordering of the links, say $1, \ldots, |\mc E|$. Given 
$y^{(k)}$, $x^{(k+1)}$ is computed as follows. \kscomment{(work in progress ...)}
%Compute $x^{(k+1)}_{|\mc E|}(t)$ and  in the \kscomment{usual way}, and then the capacity function of other links  




==> steady-state-single-link-old.tex <==
\section{Steady State Computation for a Single Link}
\label{sec:steady-state-single-link}

Let $y_i(t)$ be the cumulative inflow into link $i \in \mc E$. Referring to \eqref{eq:flow-dynamics}, this quantity is given by $y_i(t):=\lambda_i(t) + \sum_j R_{ji} z_j(t-\delta_{ji})$. For an isolated link, which is what we consider in this section, $y_i(t)=\lambda_i(t)$. It is easy to see that $x_i^*(t) \equiv 0$ if $y_i(t) \leq c_i(t)$ for all $t \in [0,T]$. In order to avoid such trivialities, we assume that the measure of the set $\setdef{t \in [0,T]}{y_i(t) > c_i(t)}$ is non-zero.
%\begin{assumption}
%\label{ass:non-triviality-condition}
%The measure of the set $\setdef{t \in [0,T]}{y_i(t) > c_i(t)}$ is non-zero.
%\end{assumption}



The key in our approach is a finite-dimensional representation of $z^*_i(t)$, for given $y_i(t)$ and $c_i(t)$. The representation will be in terms of the time instants when the queue length $x^*_i(t)$ transitions between zero and positive values. 

We implicitly assume the following \kscomment{throughout this and the next section} to avoid cumbersome technicalities in stating our formal approach.

\ksmargin{check if the definition of piecewise continuity necessarily implies finitely many points of discontinuity}
\begin{assumption}
\label{ass:continuity}
For all $i \in \mc E$, the external arrival rate $\lambda_i(t)$ and saturated capacity function $c_i(t)$ are both piecewise continuous. 
\end{assumption}


\begin{definition}[Transition Points]
\label{def:transition-points}
Let $\{\gamma_i^1, \ldots, \gamma_i^L\}$ be the times in $[0,T]$ when the queue length transitions from being positive to being zero, and let $\{\alpha_i^1, \ldots, \alpha_i^L\}$ be the times in $[0,T]$ when the queue length transitions from being zero to being positive. We choose the convention that 
\begin{equation}
\label{eq:gamma-alpha-ordering}
0 \leq \gamma_i^1 < \alpha_i^1 < \ldots < \gamma_i^L < \alpha_i^L \leq T
\end{equation}
\end{definition}


%These transition points are formalized in Algorithm~\ref{alg:transition-points}. 
%
%\begin{algorithm}[htb!]
%\Input {Link $i$ with $T$-periodic cumulative inflow and flow capacity functions $y_i(t)$ and $c_i(t)$ respectively. Let $x_i^*(t)$ and $z^*_i(t)$ denote the steady-state trajectories (cf. Theorem~\ref{thm:globally-attractive-existence}).}
%\Output{ $\gamma_i(y_i,c_i)=\left\{\gamma_i^{1}, \ldots,\gamma_i^{L} \right\}$ and $ \alpha_i(y_i,c_i)=\left\{{\alpha}_i^{1}, \ldots, \alpha_i^{L} \right\}$ }
%\textbf{initialization}:  $\gamma_i^1:=\min \setdef{s \in [0,T]}{x_i^*(s)=0}$; 
%$\alpha_i^1:=\max \setdef{s \in [\gamma_i^1,T]}{x_i^*(t)=0 \, \, \, \forall \, t \in [\gamma_i^1,s]}$; 
%$\ell=2$ \; 
%\While{ $\exists \, s \in (\alpha_i^{\ell-1},T]$ such that $x_i^*(s)=0$}{
%$\gamma^{\ell}_i := \min \setdef{s \in (\alpha_i^{\ell-1},T]}{ x^*_i(s)=0}$\; 
%%     $ \left(w^{u}_{ \mathcal{E}_{1}^{(k)}}\right)^{(k+1)} =  w^{u}_{i} $, $ \left(c_{ \mathcal{E}_{1}^{(k)}}^{l} \right)^{(k+1)} = \left(c_{ \mathcal{E}_{1}^{(k)}}^{l} \right)^{(k)} $, $ \left(c_{ \mathcal{E}_{1}^{(k)}}^{u}\right)^{(k+1)} = \left(c_{ \mathcal{E}_{1}^{(k)}}^{u}\right)^{(k)} $,  \;
%${\alpha}_i^{\ell}:=\max \setdef{s \in \left(\gamma_i^{\ell}, T \right]}{x^*_i(t)=0 \, \, \, \forall \, t \in [\gamma_i^{\ell},s]}$\;
%   $\ell = \ell+1 $\;
%  %${\gamma}_i^{\ell}(y_i,c_i):=\min \setdef{s \in [{\alpha}_i^{\ell-1}, T]}{x^*_i(s)=0}$
%   }
%   $L:=\ell-1$
%   
%   \textbf{postprocessing}: 
%   
%   \For{$\ell=1:L$}{
%   \If{$\gamma_i^{\ell}=\alpha_i^{\ell}$}{remove $\gamma_i^{\ell}$ and $\alpha_i^{\ell}$ from $\gamma_i$ and $\alpha_i$ respectively}
%   update $L$ to be the new length of $\gamma_i$ and $\alpha_i$ }
%%solve $ \mathbf{P} $ and obtain $ \nu^{*}( \mathcal{G}) = \nu^{*}\left( \mathcal{G}^{(k)}, \left(w_{ \mathcal{E}^{(k)}}^{l}\right)^{(k)}, \left(w_{ \mathcal{E}^{(k)} }^{u}\right)^{(k)},  \left(c_{ \mathcal{E}^{(k)}}^{l}\right)^{(k)}, \left(c_{ \mathcal{E}^{(k)} }^{u}\right)^{(k)}, p_{0} \right) $ \;
%%\Return{$\nu^{*}( \mathcal{G}) $}
%\caption{Definition of Transition Points.}
%\label{alg:transition-points}
%\end{algorithm}

\begin{remark}
%\begin{enumerate}
%\item 
For a given $y_i(t)$ and $c_i(t)$, Theorem~\ref{thm:globally-attractive-existence} implies uniqueness of resulting $(x^*,z^*)$, and hence of 
$\{\gamma_i^1, \ldots, \gamma_i^L\}$ and $\{\alpha_i^1, \ldots, \alpha_i^L\}$. 
%
%
%The uniqueness of $\gamma_i$ and $\alpha_i$ for given $y_i(t)$ and $c_i(t)$ is guaranteed by Theorem~\ref{thm:existence-uniqueness}. 
%\item The while loop in Algorithm~\ref{alg:transition-points} ensures that $\alpha_i^{\ell-1}<\gamma_i^{\ell}$ for $\ell \in \{2, \ldots, L\}$. The postprocessing step implies that $\gamma_i^{\ell} \neq \alpha_i^{\ell}$ for all $\ell \in \until{L}$. Therefore, collectively, we have
%\begin{equation}
%\label{eq:gamma-alpha-ordering}
%0 \leq \gamma_i^1 < \alpha_i^1 < \ldots < \gamma_i^L < \alpha_i^L \leq T
%\end{equation}
%\end{enumerate}
\end{remark}

\ksmargin{change Figure~\ref{fig:transition-points} to show multiple transition points}
\kscomment{Figure~\ref{fig:transition-points}} illustrates the transition points for a sample scenario.

%\ksmargin{what is the difference between left and right hand side of Fig~\ref{fig:transition-points} ? the figure also looks incomplete}
\begin{figure}[htb!]
\begin{center}				
\includegraphics[width=2.52in,angle=0]{../results/BW_example.pdf} 
\end{center}
\caption{ Illustration of transition points, and negative/positive sets.}
\label{fig:transition-points}
\end{figure}

$z^*(t)$ can be expressed in terms of the transition points as:
%\begin{equation}
\begin{equation}
\label{eq:zi-def}
%\begin{split}
z^*_i(t) = c_i(t) \onebf_{[0,\gamma^1_i)} + \sum_{\ell=1}^{L} y_i(t) \onebf_{[\gamma_i^{\ell},{\alpha}_i^{\ell}]} + \sum_{\ell=1}^{L-1} c_i(t) \onebf_{({\alpha}_i^{\ell},\gamma_i^{\ell+1})}   + c_i(t) \onebf_{(\alpha_i^L,T]}
%\end{split}
\end{equation}
Moreover, given the transition points, $x_i^*(t)$ is given by:
\begin{equation}
\label{eq:xi-def}
x_i^*(t) = \begin{cases}
0, & t \in [\gamma_i^{\ell}, \alpha_i^{\ell}], \, \ell \in \until{L} \\
\int_{\alpha_i^{\ell}}^t \left(\lambda_i(s) - c_i(s) \right) \, ds, & t \in [\alpha_i^{\ell}, \gamma_i^{\ell}], \, \ell \in \until{L-1}, \, \, \& \, \, t \in [\alpha_i^L,T] \\
x_i(T) + \int_0^t \left(\lambda_i(s) - c_i(s) \right) \, ds, & t \in [0,\gamma_i^1]
\end{cases}
\end{equation}

\begin{remark}
\label{rem:single-transition-point-sufficiency}
The knowledge of a single element in $\{\gamma_i^1, \ldots, \gamma_i^L\}$ or $\{\alpha_i^1, \ldots, \alpha_i^L\}$ is sufficient to determine the other transition points, by direct integration of $\lambda_i(t)-c_i(t)$. This would in turn then also determine $(x_i^*,z_i^*)$ according to \eqref{eq:xi-def} and \eqref{eq:zi-def}. \kscomment{However, our method relies on simultaneous computation of all the transition points.}
\end{remark}

%\end{equation}
\ksmargin{is this statement necessary ?}
\kscomment{\eqref{eq:zi-def} implies that $z_i^*(t)$ is left continuous at $\gamma_i^{\ell}$, $\ell \in \until{L}$, and right continuous at $\alpha_i^{\ell}$, $\ell \in \until{L}$}.
In order to construct an iterative procedure to compute $\gamma_i$ and $\alpha_i$, we need the notion of \emph{negative} and \emph{positive} sets. 
\begin{definition}[Negative and Positive Sets]
\label{def:negative-positive-sets}
Let $\{B_i^1, \ldots, B_i^{M_i^b}\}$ be contiguous subsets of $[0,T]$ of non-zero size in which $y_i(t) < c_i(t)$, and let $\{W_i^1, \ldots, W_i^{M_i^w}\}$ be contiguous subsets of $[0,T]$ in which $y_i(t) > c_i(t)$. 
\end{definition}

\begin{remark}
\begin{enumerate}
\item It is straightforward to see that $M_i^b \geq 1$ and $M_i^w \geq 1$.
%The stability condition in \eqref{eq:stability-condition} implies that $M_i^b \geq 1$. Assumption~\ref{ass:non-triviality-condition} that $M_i^r \geq 1$.
\item The sets $\{B_i^1, \ldots, B_i^{M_i^b}\}$ and $\{W_i^1, \ldots, W_i^{M_i^w}\}$ do not necessarily form a partition of $[0,T]$. In particular, they exclude points where $y_i(t)=c_i(t)$. 
\end{enumerate}
\end{remark}

The following proposition gives an inclusion relationship between the transition points and the positive/negative sets.

\begin{proposition}
\label{prop:transition-neg-pos-inclusion}
Consider a link $i$ with flow capacity function $y_i(t)$ and capacity function $c_i(t)$. Let the transition points and negative/positive sets be given by Definitions~\ref{def:transition-points} and \ref{def:negative-positive-sets} respectively. Then, 
\begin{equation*}
\label{eq:simple-inclusion}
\{\gamma_i^1, \ldots, \gamma_i^L, \alpha_i^1, \ldots, \alpha_i^L\} \subset \{\overline{B}_i^1, \ldots, \overline{B}_i^L\} \cup \{\overline{W}_i^1, \ldots, \overline{W}_i^L\} \cup \{0,T\}
\end{equation*}
where we recall that $\overline{B}_i^{\ell}$and $\overline{W}_i^{\ell}$ denote the closures of $B_i^{\ell}$ and $W_i^{\ell}$ respectively, for $\ell \in \until{L}$. 
\end{proposition}
\begin{proof}
Assume, by contradiction, that there exists $\ell \in \until{L}$ and $[\tau_1,\tau_2] \subset [0,T]$ with 
$y_i(t)-c_i(t)=0$ for all $t \in [\tau_1,\tau_2]$, such that $\alpha_i^{\ell} \in (\tau_1,\tau_2) \subset [0,T]$, with $\tau_2 > \tau_1>0$. The last inequality here follows from \eqref{eq:gamma-alpha-ordering}. If $\ell < L$, then 
there exists a sufficiently small $\epsilon>0$ so that $\alpha_i^{\ell} + \epsilon < \min \{\tau_2, \gamma_i^{\ell+1}\}$, and hence $x_i(\gamma_i^{\ell+1})=0$, contradicting $x_i(\gamma_i^{\ell+1})>0$. Similar argument can be used for $\ell=L$, and similar procedure can be repeated for proving the claim for $\gamma_i^{\ell}$.
%
%
%$\gamma_i^{\ell} \in (\tau_1,\tau_2)$ (the proof for $\alpha_i^{\ell}$ is similar). This implies that there exists a sufficiently small $\epsilon > 0$ such that $\gamma_i^{\ell} - \epsilon > \max \{\tau_1, \alpha_i^{\ell-1}\}$. This implies $x(\gamma_i^{\ell} - \epsilon) = 0$, contradicting $\gamma_i^{\ell} - \epsilon > \alpha_i^{\ell-1}$.
\end{proof}

In the next result, we sharpen Proposition~\ref{prop:transition-neg-pos-inclusion} by providing a tighter inclusion, which will then readily lead to a procedure to compute the transition points. 
%provide a tighter characterization of $\{\gamma_i^{\ell},\alpha_i^{\ell}\}$, $\ell \in \until{L}$, which facilitates their computation. 
In preparation for this next result, for $s_1, s_2 \in [0,T]$, let
$$
C_i(s_1,s_2):=\int_{s_1}^{s_2} c_i(t) \, dt, \qquad 
Y_i(s_1,s_2):=\int_{s_1}^{s_2} y_i(t) \, dt
$$

In preparation for the next result, let $\overline{B}_i^{k}=[\underline{b}_i^{k},\bar{b}_i^{k}]$, $k \in \until{M_i^b}$ and $\overline{W}_i^{k}=[\underline{w}_i^{k},\bar{w}_i^{k}]$, $k \in \until{M_i^w}$.

\begin{proposition}
\label{prop:main-computation}
Consider a link $i$ with external inflow $y_i(t)$ and saturated capacity function $c_i(t)$. Let the transition points and positive/negative sets be given by Definitions~\ref{def:transition-points} and \ref{def:negative-positive-sets} respectively. \kscomment{If $\gamma_i^1 > 0$ or $\alpha_i^L < T$,\footnote{\kscomment{It is straightforward to see from Definition~\ref{def:transition-points}, and especially from \eqref{eq:gamma-alpha-ordering},  that either $\gamma^1>0$ or $\alpha^L<T$.}}} then the following hold true:
\begin{enumerate}
\item[(I)] there exists a strictly increasing $\map{k_\alpha}{\until{L}}{\until{M_i^w}}$ such that $\alpha_i^{\ell} = \underline{w}_i^{k_{\alpha}(\ell)}$ for all $\ell \in \until{L}$;
\item[(II)] there exists a strictly increasing $\map{k_{\gamma}}{\until{L}}{\until{M_i^b}}$ such that $\gamma_i^{\ell} \in \left(\underline{b}_i^{k_{\gamma}(\ell)},\bar{b}_i^{k_{\gamma}(\ell)}\right]$ for all $\ell \in \until{L}$.
\end{enumerate} \ksmargin{are \eqref{eq:y=c} and \eqref{eq:kb-def} used anywhere ?}
Moreover, for all $\ell \in \until{L}$,
\begin{equation}
\label{eq:y=c}
y_i(t) \leq c_i(t), \qquad \forall t \in \left(\bar{b}_i^{k_{\gamma}(\ell)}, \underline{w}_i^{k_{\alpha}(\ell)} \right) \, 
\end{equation}
and, for all $\ell \in \left \{2, \ldots, L \right \}$,
\begin{equation}
\label{eq:kb-def}
k_{\alpha}(\ell)=\argmin \left \{j \in \{k_{\alpha}(\ell-1)+1, \ldots, M_i^w\} \, \Big | \, Y_i({\alpha}_i^{\ell-1},\underline{w}_i^{j}) \leq C_i({\alpha}_i^{\ell-1},\underline{w}_i^{j}) \right\}
\end{equation}
\end{proposition}
\begin{proof} 
We drop the subscript $i$ for brevity in notation. 
For claims (I) and (II), the strictly increasing property of $k_{\alpha}$ and $k_{\gamma}$, if they exist, are straightforward; we provide a proof for existence. 

Assume, by contradiction, that there exists $\ell  \in \until{L}$  such that  ${\alpha}^{\ell} \notin \{\underline{w}^{1}, \ldots, \underline{w}^{M^w}\}$. Let $$k_1:=\max \setdef{k \in \until{M^w}}{\underline{w}^k < \alpha^{\ell}}$$ if it exists, and is equal to zero otherwise. Similarly, let $k_2:=\max \setdef{k \in \until{M^b}}{\underline{b}^k \leq \alpha^{\ell}}$, if it exists, and is equal to zero otherwise. Since $k_1$ and $k_2$ can not both be equal to zero, we have $k_1 \neq k_2$. Therefore, consider the following cases, where we use the convention that $\underline{w}^0=0=\underline{b}^0$: 
\begin{enumerate}
%\item \underline{$k^r=k^b=0$}: \kscomment{(this contradicts Proposition~\ref{prop:transition-neg-pos-inclusion})}
\item $\underline{w}^{k_1} < \underline{b}^{k_2}$: 
From the definition of $k_1$, we have (i) $\alpha^{\ell} \in \left[\underline{b}^{k_2}, \underline{w}^{k_1+1}\right)$ if $k_1 < M^w$, or (ii) $\alpha^{\ell} \in \left[\underline{b}^{k_2}, T\right]$ otherwise. In case (i), $\exists \, \epsilon > 0$ such that $\alpha^{\ell} + \epsilon < \min\{\underline{w}^{k_1+1},\gamma^{\ell+1}\}$, if $\ell < L$, or $\alpha^{\ell} + \epsilon < \min\{\underline{w}^{k_1+1},T\}$ if $\ell=L$ (recall our assumption that $\alpha^{\ell} < T$). In both cases, we have $y(t)-z(t)=y(t)-c(t) \leq 0$ for all 
$t \in [\alpha^{\ell},\alpha^{\ell}+\epsilon]$.Similar argument holds true for case (ii). Therefore, 
%
%\kscomment{Proposition~\ref{prop:transition-neg-pos-inclusion} then implies that $\alpha^{\ell} \in \left[\underline{b}^{k^b}, \bar{b}^{k^b}\right]$.} Therefore, $\exists \, \epsilon >0$ such that $\alpha^{\ell} + \epsilon < \min\{\underline{b}^{k^b},\gamma^{\ell+1}\}$, if $\ell < L$, or $\alpha^{\ell} + \epsilon < \min\{\underline{r}^k,T\}$ if $\ell=L$ (recall our assumption that $\alpha^{\ell} < T$), which implies that $y(t) < c(t)$ for all $t \in [\alpha^{\ell},\alpha^{\ell}+\epsilon]$. Therefore, 
$ 
x(\alpha^{\ell} + \epsilon)= x(\alpha^{\ell} ) + \int_{\alpha^{\ell}}^{\alpha^{\ell}+\epsilon} (y(t)-c(t)) \, dt \leq x(\alpha^{\ell}) = 0
%Y_i( \alpha_i^{(k)} , \alpha_i^{(k)} + \epsilon_i ) - C_i( \alpha_i^{(k)} , \alpha_i^{(k)} + \epsilon_i )
$
which is in contradiction to $x(\alpha^{\ell}+\epsilon)>0$, since $\alpha^{\ell}+\epsilon \in \left(\alpha^{\ell}, \gamma^{\ell+1} \right)$ if $\ell < L$, or $\alpha^{\ell}+\epsilon \in \left(\alpha^{L}, T \right)$ otherwise. 

\item $\underline{b}^{k_2} < \underline{w}^{k_1}$: The definitions of $k_1$ and $k_2$ imply that $\alpha^{\ell} \in \left(\underline{w}^{k_1}, \bar{w}^{k_1}\right]$. Therefore, $\exists \, \epsilon >0$ such that $\alpha^{\ell} - \epsilon > \max\{\underline{w}^{k_1}, \gamma^{\ell}\}$, which implies that $y(t)>c(t)$ for all $t \in [\alpha^{\ell}-\epsilon,\alpha^{\ell}]$. Therefore, 
%\begin{align*}
$x(\alpha^{\ell}) =x(\alpha^{\ell}-\epsilon) + \int_{\alpha^{\ell}-\epsilon}^{\alpha^{\ell}} (y(t)-z(t)) \, dt  = \int_{\alpha^{\ell}-\epsilon}^{\alpha^{\ell}} (y(t)-z(t)) \, dt  > \int_{\alpha^{\ell}-\epsilon}^{\alpha^{\ell}} (c(t)-z(t)) \, dt \geq 0$, 
%\end{align*}
which contradicts $x(\alpha^{\ell})=0$.
\end{enumerate}
This establishes claim (I) in the proposition. 

In order to establish claim (II), following Proposition~\ref{prop:transition-neg-pos-inclusion}, it suffices to show that, for all $\ell \in \until{L}$, (i) $\gamma^{\ell} \notin [\underline{w}^k,\bar{w}^k]$ for all $k \in \until{M^w}$, and (ii) $\gamma^{\ell} \neq \underline{b}^k$ for all $k \in \until{M^b}$. 

In order to show (i), assume by contradiction that there exists $k \in \until{M^w}$ such that $\gamma^{\ell} \in [\underline{w}^k,\bar{w}^k]$. Choose $\epsilon > 0$ such that $\gamma^{\ell} + \epsilon < \min \left\{\alpha^{\ell}, \bar{w}^{k} \right \}$. Therefore, for all $t \in [\gamma^{\ell},\gamma^{\ell}+\epsilon]$, we have that $y(t)>c(t)$, which implies that 
%\begin{align*}
$x(\gamma^{\ell}+ \epsilon) = x(\gamma^{\ell}) + \int_{\gamma^{\ell}}^{\gamma^{\ell} + \epsilon} (y(t)-z(t)) \, dt  \geq x(\gamma^{\ell}) + \int_{\gamma^{\ell}}^{\gamma^{\ell} + \epsilon} (y(t)-c(t)) \, dt  > x(\gamma^{\ell}) = 0$
%\end{align*}
contradicting $\gamma^{\ell} + \epsilon < \alpha^{\ell}$.

(i) establishes that $\gamma^{\ell} \in [\underline{b}^k,\bar{b}^k]$ for some $k \in \until{M^b}$. Assume by contradiction that $\gamma^{\ell} = \underline{b}^k$ for some $k \in \until{M^b}$. One can then choose a sufficiently small $\epsilon>0$ such that $\gamma^{\ell} - \epsilon > \alpha^{\ell-1}$ if $\ell > 1$, or $\gamma^{\ell} - \epsilon > 0$ if $\ell=1$ (recall our assumption that $\gamma^1>0$), and that $y(t) - c(t) \geq 0$ for all $t \in [\gamma^{\ell}-\epsilon, \gamma^{\ell}]$. However, this implies that 
%\begin{align*}
$x(\gamma^{\ell}-\epsilon) = x(\gamma^{\ell}) - \int_{\gamma^{\ell} - \epsilon}^{\gamma^{\ell}} (y(t) - z(t)) \, dt  = x(\gamma^{\ell}) - \int_{\gamma^{\ell} - \epsilon}^{\gamma^{\ell}} (y(t) - c(t)) \, dt \leq x(\gamma^{\ell}) = 0$, 
%\end{align*}
contradicting $x(\gamma^{\ell} - \epsilon) > 0$. This concludes proof of claim (II).

In order to prove \eqref{eq:y=c}, assume by contradiction and utilizing Assumption~\ref{ass:continuity} that there exists $[t_1,t_2] \in \left(\bar{b}^{k_\gamma(\ell)}, \underline{w}^{k_{\alpha}(\ell)} \right)$ such that $y(t) > c(t)$ for all $t \in [t_1,t_2]$, which then implies that $x(t_2)>0$, thereby contradicting $t_2 < \alpha^{\ell}$. 

In order to prove \eqref{eq:kb-def}, observe that 
%\begin{subequations}
%\begin{align}
\begin{equation}
\label{eq:bisection}
\begin{split}
Y(\alpha^{\ell-1},t) - C(\alpha^{\ell-1},t) & > 0, \qquad t \in (\alpha^{\ell-1},\gamma^{\ell}) \\
Y(\alpha^{\ell-1},\gamma^{\ell}) - C(\alpha^{\ell-1},\gamma^{\ell}) & = 0 \\
Y(\alpha^{\ell-1},t) - C(\alpha^{\ell-1},t) & < 0, \qquad t \in (\gamma^{\ell},\bar{b}^{k_{\gamma}(\ell)}] \\
Y(\alpha^{\ell-1},t) - C(\alpha^{\ell-1},t) & \leq 0, \qquad t \in [\bar{b}^{k_{\gamma}(\ell)},\underline{w}^{k_{\alpha}(\ell)}]
\end{split}
\end{equation}
%\end{align}
%\end{subequations}
where the first relationship follows from $x(t)>0$, and hence $z(t)=c(t)$ for all $t \in (\alpha^{\ell-1},\gamma^{\ell})$; and the fourth relationship follows from the second and third relationship and \eqref{eq:y=c}. \eqref{eq:kb-def} then follows by noting that \eqref{eq:y=c} also implies $[\gamma^{\ell}, \underline{w}^{k_{\alpha}(\ell)}) \cap \{\underline{w}^1, \ldots, \underline{w}^{M_w}\} = \emptyset$.
\end{proof}

\kscomment{
\begin{remark} 
If $\alpha_i^L=T$ (respectively, $\gamma_i^1=0$), then claim I (respectively, claim II) in Proposition~\ref{prop:main-computation} holds true for $\ell \in \until{L-1}$. 
\end{remark}
}


\eqref{eq:kb-def} gives a sequential approach to determine $\{k_{\alpha}(2), \ldots, k_{\alpha}(L)\}$, once $k_{\alpha}(1)$ is known. \kscomment{We now give a simple procedure to determine $\alpha_i^L$.}
%Algorithm~\ref{alg:gamma-1-computation} describes a procedure to determine $k_{\alpha}(1)$ iteratively. This in turn, combined with Proposition~\ref{prop:main-computation}, will then give all the necessary ingredients for determining the transition points for given $y_i(t)$ and $c_i(t)$. 
%%The steps are formalized in Algorithm~\ref{alg:gamma-1-computation}. 
%In preparation for the algorithm, 
Motivated by \eqref{eq:y=c}, let $\mc W_i^{\alpha} := \left\{\underline{w}_i^{k_1}, \ldots,  \underline{w}_i^{k_m}\right \}$ be such that $k_1=1$, and, for $j \in \{2, \ldots, m\}$, 
%\begin{equation}
%\label{eq:M-def}
%k_j = \argmin \left \{ind \in \{k_{j-1}+1, \ldots, M^w\} \, \Big | \, [\underline{w}_i^{ind-1},\underline{w}_i^{ind}] \cap \{\underline{b}_i^1, \ldots, \underline{b}_i^{M_i^b}\} \neq \emptyset \right\}
%\end{equation}
%\begin{equation}
\ksmargin{this may still give $\gamma_i^{\ell}=\alpha_i^{\ell}$}
\begin{multline}
\label{eq:M-def}
k_j = \argmin \Big \{ind \in \{k_{j-1}+1, \ldots, M^w\} \, \Big | \, \exists \, p \in \until{M_i^b} \text{ s.t. } \bar{b}_i^p \in [\underline{w}_i^{ind-1},\underline{w}_i^{ind}] \\  \& \quad Y_i(\underline{w}_i^{ind-1},\bar{b}_i^p) \kscomment{\leq} C_i(\underline{w}_i^{ind-1},\bar{b}_i^p) \Big \}
\end{multline}
%\end{equation}
where $m$ is implicitly defined to be the maximum value of $k_j$, when the set over which $\argmin$ is taken in \eqref{eq:M-def} is empty. 
The next result sharpens Proposition~\ref{prop:main-computation} to the point where it can be used directly to compute $\alpha_i^L$, and hence the rest of the transition points, as per Remark~\ref{rem:single-transition-point-sufficiency}. 


\begin{proposition}
\label{prop:gamma-1-computation-correctness}
Consider a link $i$ with inflow function $y_i(t)$ and capacity function $c_i(t)$, and the corresponding set $\mc W_i^{\alpha}$ defined via \eqref{eq:M-def}. Then $\{\alpha_i^1, \ldots, \alpha_i^L\} \subseteq \mc W_i^{\alpha}$, and, in particular, 
\begin{equation}
\label{eq:alpha-exact-expr}
\alpha_i^{\ell}=\underline{w}_i^{k_m+\ell-L}, \qquad \ell \in \until{L}
\end{equation}
\end{proposition}
\begin{proof}
%For brevity in notation, we drop the subscript $i$ from various quantities. Proposition~\ref{prop:main-computation} implies that $\{\alpha^1, \ldots, \alpha^L\} \in \{\underline{w}^1, \ldots, \underline{w}^{M^w}\} \supset \mc W^{\alpha}$. We first show that $\alpha^1 \in \mc W^{\alpha}$. This is trivially true if $\alpha^1 = \underline{w}^{k_1}$. If $\alpha^1 > \underline{w}^{k_1}$ (recall that $k_1=1$), then we prove by contradiction. Assume that $\alpha^1 = \underline{w}^{k} \in \{\underline{w}^1, \ldots, \underline{w}^{M^w}\} \setminus \mc W^{\alpha}$, and let $\hat{k}$ be the largest element in $\{k_1, \ldots, k_m\}$ such that $\alpha^1 = \underline{w}^{k_{\alpha}(1)}> \underline{w}^{\hat{k}}$. If $\gamma^1 < \underline{w}^{\hat{k}}$ \kscomment{then $\alpha^1=\underline{w}^{\hat{k}}$} which would be a contradiction. Therefore, $\underline{w}^{\hat{k}} < \gamma^1 < \alpha^1$, which would imply that $x(\underline{w}^{\hat{k}})+ Y(\underline{w}^{\hat{k}},\bar{b}^{k_{\gamma}(1)})-C(\underline{w}^{\hat{k}},\bar{b}^{k_{\gamma}(1)}) \leq 0$, which in turn implies that $Y(\underline{w}^{\hat{k}},\bar{b}^{k_{\gamma}(1)})-C(\underline{w}^{\hat{k}},\bar{b}^{k_{\gamma}(1)}) \kscomment{\leq 0}$. However, referring to \eqref{eq:M-def}, this would imply $k_{\alpha}(1) \in \{k_1, \ldots, k_m\}$, giving a contradiction. 
%
Fix some $\ell \in \until{L}$. Proposition~\ref{prop:main-computation} implies that $\alpha^{\ell}=\underline{w}^{k_{\alpha}(\ell)}$. Assume by contradiction that $k_{\alpha}(\ell) \notin \{k_1, \ldots, k_m\}$. Let $\hat{k}$ be the largest element in $\{k_1, \ldots, k_m\}$ which is less than $k_{\alpha}(\ell)$. Since $k_1=1$ (by definition), $\hat{k} \geq 1$ is well-defined. If $\gamma^{\ell} < \underline{w}^{\hat{k}}$, then $\alpha^{\ell}=\underline{w}^{\hat{k}}$, giving a contradiction. Therefore, $\underline{w}^{\hat{k}} < \gamma^{\ell} < \alpha^{\ell}$, which would imply $x(\underline{w}^{\hat{k}})+ Y(\underline{w}^{\hat{k}},\bar{b}^{k_{\gamma}(\ell)})-C(\underline{w}^{\hat{k}},\bar{b}^{k_{\gamma}(\ell)}) = x(\underline{w}^{\hat{k}})+ Y(\underline{w}^{\hat{k}},\gamma^{\ell})-C(\underline{w}^{\hat{k}},\gamma^{\ell}) + Y(\gamma^{\ell},\bar{b}^{k_{\gamma}(\ell)}) - C(\gamma^{\ell},\bar{b}^{k_{\gamma}(\ell)}) = Y(\gamma^{\ell},\bar{b}^{k_{\gamma}(\ell)}) - C(\gamma^{\ell},\bar{b}^{k_{\gamma}(\ell)}) \leq 0$. This in turn would give $Y(\underline{w}^{\hat{k}},\bar{b}^{k_{\gamma}(\ell)})-C(\underline{w}^{\hat{k}},\bar{b}^{k_{\gamma}(\ell)}) \leq - x(\underline{w}^{\hat{k}}) \leq 0$. However, referring to \eqref{eq:M-def}, this would imply $k_{\alpha}(\ell) \in \{k_1, \ldots, k_m\}$, giving a contradiction. 

In order to prove \eqref{eq:alpha-exact-expr}, observe that if $\alpha^{\ell}=\underline{w}^{k_j}$ for some $\ell \in \until{L-1}$, then $\alpha^{\ell+1}=\underline{w}^{k_j+1}$. If $\alpha^L=T$, then it is easy to see that $\alpha^L=\underline{w}^{k_m}$. If $\alpha^L<T$, then assume $k_{\alpha}(L)=k_{m_1}$ with  $m_1<m$. Therefore, \eqref{eq:M-def} implies that $\underline{w}^{k_{m_1+1}} > \alpha^L$ is a point where the queue length transitions from being zero to being positive, giving a contradiction. 
\end{proof}

\begin{remark}
\label{rem:alpha-L-to-all-transition-points}
Note that since $L$ is not known, \eqref{eq:alpha-exact-expr} can not be used to compute all $\alpha_i^{\ell}$, $\ell \in \until{L}$. However, \eqref{eq:alpha-exact-expr} readily gives us the value of $\alpha_i^{L}$, which then gives $x_i(0)=Y_i(\alpha_i^L,T)-C_i(\alpha_i^L,T)$. Thereafter, the rest of the transition points, i.e., $\{\gamma_i^1, \ldots, \gamma_i^L\}$ and $\{\alpha_i^1, \ldots, \alpha_i^{L-1}\}$, \kscomment{can be easily computed, as noted in Definition~\ref{def:transition-points} and Remark~\ref{rem:single-transition-point-sufficiency}}.
\end{remark}

\ksmargin{need to add more details for $\mc F_x(y_i,c_i)$}
Recall from \eqref{eq:zi-def} that the steady-state link outflows for a single link corresponding to periodic cumulative inflow $y_i(t)$ and capacity function $c_i(t)$ can be written in terms of the transition points. Let this relationship be denoted as $z_i=\mc F_z(y_i,c_i)$. \kscomment{Similarly, let $x_i=\mc F_x(y_i,c_i)$ denote the procedure by which the steady-state queue length for link $i$ can be written in terms of the transitions points corresponding to $y_i$ and $c_i$.} The following corollary to Lemmas~\ref{lem:monotonicity} and \ref{lem:attractivity} will be useful for extending our computations from a single link to the network setting in Section~\ref{sec:steady-state-network}.
\begin{corollary}
\label{cor:input-output-monotonicity}
Consider a link $i \in \mc E$ with $T$-periodic saturated capacity function $c_i(t)$.
Let $y_i(t)$ and $y_i'(t)$ be $T$-periodic inflow functions, both satisfying the stability condition in Definition~\ref{def:stability}, and $y_i(t) \leq y'_i(t)$ for all $t \in [0,T]$. If the corresponding steady state $T$-periodic queue lengths are $x^*_i(t)$ and ${x^*}_i'(t)$ respectively, and the steady state $T$-periodic link outflows are $z^*_i(t)$ and ${z^*}'_i(t)$ respectively, then $x^*_i(t) \leq {x^*}'_i(t)$ and $z^*_i(t) \leq {z^*}'_i(t)$ for all $t \in [0,T]$.
\end{corollary}
\begin{proof}
Let $(x(t),z(t))$ and $(x'(t),z'(t))$ be the system trajectories for the two systems, both starting from initial condition $x_0$. Lemma~\ref{lem:monotonicity} implies that $x'(t) \geq x(t)$ and $z'(t) \geq z(t)$ for all $t \geq 0$. On the other hand, Theorem~\ref{thm:globally-attractive-existence} implies that $(x(t),z(t))$ and $(x'(t),z'(t))$ converge to $T$-periodic trajectories $(x^*(t),z^*(t))$ and $({x^*}'(t),{z^*}'(t))$ respectively. Combining these facts gives the desired result. 
\end{proof}

\begin{algorithm}[htb!]
\Input {$T$- periodic inflow function $\lambda_i(t)$ and periodic capacity function $c_i(t)$}
\textbf{initialization}:  $y_i(t)=\lambda_i(t)$, $t \in [0,T]$\;
compute $\alpha_i^{L}$ from \eqref{eq:alpha-exact-expr}\;
compute $x^*_i(0)= Y_i(\alpha_i^L,T)-C_i(\alpha_i^L,T)$ \;
compute $x_i^*(t)$ and $z_i^*(t)$, $t \in [0,T]$, by direct simulation of \eqref{eq:flow-dynamics}-\eqref{z-linprog} with initial condition $x_i^*(0)$ \; 
\caption{ Computation of $(x_i^*,z_i^*)$ for isolated link $i$}
\label{alg:steady-state-computation-single-link}
\end{algorithm}

